Video Violence Recognition and Localization Using a Semi-Supervised Hard Attention Model

The significant growth of surveillance camera networks necessitates scalable AI solutions to efficiently analyze the large amount of video data produced by these networks. As a typical analysis performed on surveillance footage, video violence detection has recently received considerable attention. The majority of research has focused on improving existing methods using supervised methods, with little, if any, attention to the semi-supervised learning approaches. In this study, a reinforcement learning model is introduced that can outperform existing models through a semi-supervised approach. The main novelty of the proposed method lies in the introduction of a semi-supervised hard attention mechanism. Using hard attention, the essential regions of videos are identified and separated from the non-informative parts of the data. A model's accuracy is improved by removing redundant data and focusing on useful visual information in a higher resolution. Implementing hard attention mechanisms using semi-supervised reinforcement learning algorithms eliminates the need for attention annotations in video violence datasets, thus making them readily applicable. The proposed model utilizes a pre-trained I3D backbone to accelerate and stabilize the training process. The proposed model achieved state-of-the-art accuracy of 90.4% and 98.7% on RWF and Hockey datasets, respectively.

==> response.tex <==
\section*{Reviewer Response}
\label{response}

It is our pleasure to thank the Editor-in-Chief, Dr. Binshan Lin, Associate Editor, and all the reviewers for their thoughtful and thorough comments. We have carefully considered your comments and applied the suggested changes. The revised article has improved significantly as a result of the detailed comments. Hopefully, the revised paper and reviewer responses will address all your concerns. The following sections are as follows: \hyperref[1a]{Section 1-a} and \hyperref[1b]{1-b} presents the full Editor-in-chief decision letter and authors response to Editor-in-chief. Next, \hyperref[2a]{Section 2-a} and \hyperref[2b]{2-b} address Associate Editor's comments and its corresponding responses. Finally, \hyperref[3a]{Section 3-a} and \hyperref[3b]{3-b} provides the reviewer comments, followed by the detailed response to reviewers.

\subsection*{\textbf{Section 1-a: Editorial decision letter}}
\label{1a}

Ms. Ref. No.: ESWA-D-22-02536

Title: SSHA: Video Violence Recognition and Localization Using a Semi-Supervised Hard Attention Model

Expert Systems With Applications

Dear Dr. Ehsan Nazerfard,

As Editor-in-Chief, I’m writing this editorial decision letter on your paper submission ESWA-D-22-02536. If you are interested in submitting a revised version, please read through this entire editorial decision letter carefully and take all actions seriously in order to avoid any delay in the review process of your revised manuscript submission. You need to upload a ‘Detailed Response to Reviewers’ in the EM system with the following sections while submitting the revised manuscript. Please note that the Required Sections (Section #1 - a & b, Section #2 - a & b, Section #3 - a & b) with specific Compliance Requirements (stated in this editorial decision letter) must be clearly labeled and included in the 'Detailed Response to Reviewers.’ The Required Sections must be clearly placed before the revised manuscript. NOTE: Section #1-(a) MUST contain the COMPLETE text covered in this email letter from Editor-in-Chief, rather than just only the first paragraph of this email letter from Editor-in-Chief. Please note that we will NOT admit any revised manuscript submission for further review if any of the Required Sections (i.e., Section #1 – a & b, Section #2 – a & b, Section #3 – a & b) is incomplete or any non-compliance of the ESWA authors’ guidelines in the PDF file of the revised manuscript that you approve in EM system. So you need to take both (1) Required Sections and (2) Compliance Requirements seriously to avoid any delay in the review process of your revised manuscript. The font size of the Required Sections should be consistent and readable. The Required Sections must be placed in the order listed:

REQUIRED SECTIONS:

Section #1: a) and b)

a. The entire editorial decision letter (i.e., complete text covered in this email letter) from Editor-in-Chief, and

b. your Point-to-Point responses to Editor-in-Chief in terms of (1) Required Sections and (2) Compliance Requirements.

Section #2: a) and b)

a. The entire editorial decision comments made by the Associate Editor, and

b. your Point-to-Point responses to the Associate Editor.

Section #3: a) and b)

a. The entire comments made by the Reviewers, and

b. your Point-to-Point responses to the Reviewers. Your Point-to-Point responses should be grouped by reviewers.

COMPLIANCE REQUIREMENTS:

In addition, please note that prior to admitting the revised submission to the next rigorous review process, all paper submissions must completely comply with ESWA Guide for Authors (see details at https://www.elsevier.com/journals/expert-systems-with-applications/0957-4174/guide-for-authors). These include at least the following Compliance Requirements:

A) Authorship policies - Please also note that ESWA takes authorship very seriously and all paper submissions MUST completely comply with all of the following three policies on authorship (clearly stated in the questionnaire responses in EM system) prior to a rigorous peer review process:

A)-1: The corresponding author needs to enter the full names, full affiliation with country and email address of every contributing author in EM online system. It is also mandatory that every contributing coauthor must be listed in EM at submission.

A)-2: It is mandatory that the full names, full affiliation with country and email address of every contributing author must be included in title (authorship) page of the manuscript. The first page of the manuscript should contain the title of the paper, and the full name, full affiliation with country and email address of every contributing author. The second page of the manuscript should begin with the paper abstract. Note that cover letter is not title (authorship) page.

A)-3: The authorship information in EM system must be consistent with the authorship information on the title (authorship) page of the manuscript.

B) Guidelines of reference style and reference list – Citations in the text should follow the referencing style used by the American Psychological Association (APA).

B)-1: Reference Style: Citations in the text should follow the referencing style used by the American Psychological Association. You are referred to the Publication Manual of the American Psychological Association, Sixth Edition, ISBN 978-1-4338-0561-5. APA’s in-text citations require the author’s last name and the year of publication. You should cite publications in the text, for example, (Smith, 2020). However, you should not use [Smith, 2020]. Note: There should be no [1], [2], [3], etc in your manuscript.

B)-2: Reference List:
References should be arranged first alphabetically by the surname of the first author followed by initials of the author’s given name, and then further sorted chronologically if necessary. More than one reference from the same author(s) in the same year must be identified by the letters 'a', 'b', 'c', etc., placed after the year of publication. For example, Van der Geer, J., Hanraads, J. A. J., & Lupton, R. A. (2010). The art of writing a scientific article. Journal of Scientific Communications, 163, 51–59. https://doi.org/10.1016/j.Sc.2010.00372. Note: There should be no [1], [2], [3], etc in your references list.

C) Highlights guidelines – There should be a maximum of 85 characters, including spaces, per Highlight. Please kindly read this guideline carefully - the guideline does NOT say there should be a maximum of 85 words per Highlight. It says there should be a maximum of 85 characters per Highlight. As examples, the word “impact” consists of 6 characters; the word "significance" consists of 12 characters. Only include 3 to 5 Highlights. Minimum number is 3, and maximum number is 5.

NOTE: Your paper submission will be returned to authors and will NOT be admitted to further review if the revised paper fails to completely comply with the ESWA Authorship policies, ESWA guidelines of reference style and reference list, Highlights guidelines. You need to take the Compliance Requirements seriously to avoid any delay in the review process of your revised manuscript.

The submission deadline of revised version is August 7, 2022.

Look forward to receiving your revised submission and Required Sections (i.e., Section #1 – a & b, Section #2 – a & b, and Section #3 – a & b) with Compliance Requirements in 'Detailed Response to Reviewers.'\\

With kind regards,

Dr. Binshan Lin

BellSouth Professor

Editor-in-Chief, Expert Systems with Applications

Louisiana State University Shreveport

Email: Binshan.Lin@LSUS.edu

\subsubsection*{\textbf{Associate editor comments}}

1. Reviewers agree that the manuscript contains novel elements. However, it presents some aspects that need to be solved before reconsideration.
The authors should explicitly mention the significant contributions of the manuscript. The novelty of the paper is not highlighted.
Please correct the typos and grammatical errors.
The advantages and limitations of the compared schemes in relationship with similar schemes is not clear.
Please revise the structure of the paper. It is recommendable to add in each section a couple of sentences that explain which is the purpose of the section. With this organization, the reader can clearly understand the sequence of the paper.
Under the review observations, the paper should be corrected as a major revision.

Authors need to revise paper and provide very convincing point-to-point responses according to the comments raised by the reviewers. When you revise your submission please highlight the changes you make in the manuscript by using colored text. Please note that you are not obliged to add suggested references by the reviewers. If you detect any abuse in the suggested literature, please do not hesitate to contact me.

2. Prior to the next review process, you need to completely comply with

    \quad 1) ESWA authorship policies,

    \quad 2) ESWA guidelines of reference style and reference list, and

    \quad 3) highlight guidelines.

Any non-compliance paper submission will be returned to authors. Please do take the Compliance Requirements seriously to avoid any delay in the review process of your revised manuscript.

3. Prior to the next review process, your submission needs to include each of the “Required Sections.” The Required Sections must be placed in the order listed: Section #1 – a, Section #1-b, Section #2-a, Section #2-b, Section #3-a, and Section #3-b.

Note that Section #1- a MUST contain the COMPLETE text covered in this email letter from Editor-in-Chief. Your paper submission will be returned to authors and will NOT be admitted to further review if the revised paper submission is incomplete. So please take both (1) Required Sections and (2) Compliance Requirements seriously to avoid any delay in the review process of your revised manuscript.

4. The authors need to provide explicit evidence that the manuscript was checked by a native speaker, e.g., in the revision, include difference file (from this submission to the new submission) or a certificate from professional editing.

\subsubsection*{\textbf{Reviewer comments}}

\textbf{Reviewer \#1:}

The manuscript needs an English proofreading.


\textbf{Reviewer \#2:}

In this paper, the authors proposed a semi-supervised hard attention model for video violence recognition and localization. Followings are required to be revised for the improvement of this paper.

\begin{itemize}
    \item Firstly, the paper is not organized well. You need to format your paper in accordance with the Expert Systems With Applications Journal formatting style.
    
    \item The abstract is not convincing and is disorganized, it should be refined to precisely illustrate what authors have done in this paper within 250 words. The abstract must be a concise yet comprehensive reflection of what is in your paper. Remember that the reader wants to know: 1-what is the problem. 2- why the problem is relevant 3- wants an overview of your approach. 4-need to know the results.

    \item The tense used in sentences are not consistent.

    \item The whole text should be revised since there are misuses of words.

    \item There are no citations for many sentences in this manuscript. Why? Please check.

    \item Please proof-read the whole text.

    \item The conclusions are not in accordance with the main problem originally stated.
\end{itemize}

\textbf{Reviewer \#3:}

The authors have proposed a semi-supervised hard attention model for achieving better accuracy on the violence detection task. While the paper has potential, few points needs careful evaluation.

In the process, authors have proposed a hard attention mechanism where the so called redundant information is completed removed. Can removing the background information be a substitute to having additional features? Will this approach work in other general situations? Needs discussion.

The evaluation measure is accuracy. Is this a good measure to evaluate the performance? It may be appropriate to look at classification performance for each of the classes, particularly because the classes are not of equal importance. Appropriate measures need to be used.

It is stated that Table 1 presents statistical comparison. This is misleading as the table provides some details about the data set.



\textbf{Reviewer \#5:}

This manuscript describes the implementation of a semi-supervised hard attention model (SSHA) for video violence recognition and localization on two datasets (RWF and Hockey). The topic is very interesting and has received increasing attention in recent years. Unfortunately, the presentation of the work needs better clarification, in particular, the authors largely focused on describing the characteristics of the state of the art, and little is done to provide insight regarding the description of the assumed models and their setups. In fact, the reader is not able to obtain a clear understanding or appreciation of the work carried out in this manuscript. There are many cases of an unclear definition of the terminology used throughout the manuscript, presenting big ambiguity towards the application of the models. Lacking scientific novelty is also another issue. One can easily notice that the authors merely made a simple amendment to the established techniques and source codes. Besides these concerns, the manuscript is not well structured and there is a lack of logical flow. Some specific comments are listed below.

\begin{enumerate}
    \item The abstract is vague and does not report any essential mechanism of the SSHA.
    
    \item It is not understood why the authors used BGR video frames instead of the standard RGB format. This raise two concerns: (1) Converting RGB2BGR may entail more computational time, (2) The competitor methods/models (Table 2) entirely based on RGB frames, which means that no fair comparison can been made.

    \item Most of the parameters of the Eq1 are not defined. This also applies to Eq2, 3, and 4. Further, no references to Eq1 and 2.

    \item In the subsection "3.2 Design", what is a? Why a+1 is the correct selection, also why a-1 is the wrong selection? Why +0.5?

    \item In page 6, line 22: The authors mentioned that the predefined range is application and architecture-specific. However, I do not see this range in the evaluation part of this paper.

    \item Finally, the authors presented insufficient results for violence recognition, and no "actual" results are provided for the violence localization.
\end{enumerate}

\subsection*{\textbf{Section 1-b: Response to Editor-in-Chief}}
\label{1b}

Dear Dr. Binshan Lin, thank you for your insightful and detailed comments. We have carefully considered your comments and incorporated them into the revised paper. The required sections are included in the “Response to Reviewers." Some of the applied changes include:

\begin{itemize}
    \item All authors have registered in the online editorial system using their full name, affiliation with country, and email address.
    \item The name, affiliation, and email address of all authors are mentioned on the authors' page before the abstract.
    \item The authorship information on the paper matches the ones in the online editorial system.
    \item The in-text references and the reference list completely comply with the APA referencing style.
    \item 5 highlights are included in the paper, with each highlight having less than 85 characters.
\end{itemize}

\subsection*{\textbf{Section 2-a: Associate Editor comments}}
\label{2a}

1. Reviewers agree that the manuscript contains novel elements. However, it presents some aspects that need to be solved before reconsideration.
The authors should explicitly mention the significant contributions of the manuscript. The novelty of the paper is not highlighted.
Please correct the typos and grammatical errors.
The advantages and limitations of the compared schemes in relationship with similar schemes is not clear.
Please revise the structure of the paper. It is recommendable to add in each section a couple of sentences that explain which is the purpose of the section. With this organization, the reader can clearly understand the sequence of the paper.
Under the review observations, the paper should be corrected as a major revision.

Authors need to revise paper and provide very convincing point-to-point responses according to the comments raised by the reviewers. When you revise your submission please highlight the changes you make in the manuscript by using colored text. Please note that you are not obliged to add suggested references by the reviewers. If you detect any abuse in the suggested literature, please do not hesitate to contact me.

2. Prior to the next review process, you need to completely comply with

    \quad 1) ESWA authorship policies,

    \quad 2) ESWA guidelines of reference style and reference list, and

    \quad 3) highlight guidelines.

Any non-compliance paper submission will be returned to authors. Please do take the Compliance Requirements seriously to avoid any delay in the review process of your revised manuscript.

3. Prior to the next review process, your submission needs to include each of the “Required Sections.” The Required Sections must be placed in the order listed: Section #1 – a, Section #1-b, Section #2-a, Section #2-b, Section #3-a, and Section #3-b.

Note that Section #1- a MUST contain the COMPLETE text covered in this email letter from Editor-in-Chief. Your paper submission will be returned to authors and will NOT be admitted to further review if the revised paper submission is incomplete. So please take both (1) Required Sections and (2) Compliance Requirements seriously to avoid any delay in the review process of your revised manuscript.

4. The authors need to provide explicit evidence that the manuscript was checked by a native speaker, e.g., in the revision, include difference file (from this submission to the new submission) or a certificate from professional editing.

\subsection*{\textbf{Section 2-b: Response to Associate Editor}}
\label{2b}

Dear Associate Editor, it is a pleasure to receive your valuable comments. Your suggestions have helped us improve the paper. The changes made to the paper based on your recommendations are:

\begin{enumerate}
    \item The paper is updated according to your comments:
    \begin{itemize}
        \item The novelty of the paper is now explicitly mentioned in the paper:
        
        \textbf{Abstract:} \textit{"The main novelty of the proposed method lies in the introduction of a semi-supervised hard attention mechanism…"}
        
        \textbf{Introduction, paragraph 8:} \textit{"The novelty of this study lies in the use of semi-supervised reinforcement learning techniques to create a hard attention mechanism to improve the purity of visual data to achieve state-of-the-art accuracy…"}
        
        \textbf{Conclusions and future work:} \textit{"The novelty of the SSHA model is the improvement of state-of-the-art violence detection accuracy through semi-supervised reinforcement learning techniques. SSHA achieves state-of-the-art accuracy in video violence detection by analyzing the most critical region of the video in greater depth…"}
        
        \item The paper has undergone professional proofreading by native editors. Additionally, the paper has been proofread multiple times by the authors. Hopefully, the paper's language quality has improved significantly.
        
        \item The discussion section has been majorly updated. It is dedicated to the advantages and limitations of the proposed method, including the comparison to similar methods.
        
        \item The structure of the paper is majorly updated. Many paragraphs have been rewritten, replaced, added, or removed. Each section contains an introduction paragraph now.
        
        \item As the paper has undergone major changes, and only the most important changes are highlighted to avoid confusion.
    \end{itemize}
    
    \item We have carefully studied the ESWA authorship policies, ESWA guidelines of reference style and reference list, and highlight guidelines. The author guidelines are complied with in the revised version.

    \item The required sections are included in this "response to reviewers."
    
    \item A professional native editor has edited the paper. The certificate of native English editing is included as an attachment.
\end{enumerate}

\subsection*{\textbf{Section 3-a: Reviewer comments}}
\label{3a}

\subsubsection*{\textbf{Reviewer \#1:}}

The manuscript needs an English proofreading.

\subsubsection*{\textbf{Reviewer \#2:}}

In this paper, the authors proposed a semi-supervised hard attention model for video violence recognition and localization. Followings are required to be revised for the improvement of this paper.

\begin{itemize}
    \item Firstly, the paper is not organized well. You need to format your paper in accordance with the Expert Systems With Applications Journal formatting style.
    
    \item The abstract is not convincing and is disorganized, it should be refined to precisely illustrate what authors have done in this paper within 250 words. The abstract must be a concise yet comprehensive reflection of what is in your paper. Remember that the reader wants to know: 1-what is the problem. 2- why the problem is relevant 3- wants an overview of your approach. 4-need to know the results.

    \item The tense used in sentences are not consistent.

    \item The whole text should be revised since there are misuses of words.

    \item There are no citations for many sentences in this manuscript. Why? Please check.

    \item Please proof-read the whole text.

    \item The conclusions are not in accordance with the main problem originally stated.
\end{itemize}

\subsubsection*{\textbf{Reviewer \#3:}}

The authors have proposed a semi-supervised hard attention model for achieving better accuracy on the violence detection task. While the paper has potential, few points needs careful evaluation.

In the process, authors have proposed a hard attention mechanism where the so called redundant information is completed removed. Can removing the background information be a substitute to having additional features? Will this approach work in other general situations? Needs discussion.

The evaluation measure is accuracy. Is this a good measure to evaluate the performance? It may be appropriate to look at classification performance for each of the classes, particularly because the classes are not of equal importance. Appropriate measures need to be used.

It is stated that Table 1 presents statistical comparison. This is misleading as the table provides some details about the data set.



\subsubsection*{\textbf{Reviewer \#5:}}

This manuscript describes the implementation of a semi-supervised hard attention model (SSHA) for video violence recognition and localization on two datasets (RWF and Hockey). The topic is very interesting and has received increasing attention in recent years. Unfortunately, the presentation of the work needs better clarification, in particular, the authors largely focused on describing the characteristics of the state of the art, and little is done to provide insight regarding the description of the assumed models and their setups. In fact, the reader is not able to obtain a clear understanding or appreciation of the work carried out in this manuscript. There are many cases of an unclear definition of the terminology used throughout the manuscript, presenting big ambiguity towards the application of the models. Lacking scientific novelty is also another issue. One can easily notice that the authors merely made a simple amendment to the established techniques and source codes. Besides these concerns, the manuscript is not well structured and there is a lack of logical flow. Some specific comments are listed below.

\begin{enumerate}
    \item The abstract is vague and does not report any essential mechanism of the SSHA.
    
    \item It is not understood why the authors used BGR video frames instead of the standard RGB format. This raise two concerns: (1) Converting RGB2BGR may entail more computational time, (2) The competitor methods/models (Table 2) entirely based on RGB frames, which means that no fair comparison can been made.

    \item Most of the parameters of the Eq1 are not defined. This also applies to Eq2, 3, and 4. Further, no references to Eq1 and 2.

    \item In the subsection "3.2 Design", what is a? Why a+1 is the correct selection, also why a-1 is the wrong selection? Why +0.5?

    \item In page 6, line 22: The authors mentioned that the predefined range is application and architecture-specific. However, I do not see this range in the evaluation part of this paper.

    \item Finally, the authors presented insufficient results for violence recognition, and no "actual" results are provided for the violence localization.
\end{enumerate}

\subsection*{\textbf{Section 3-b: Response to reviewers}}
\label{3b}

Thank you for your response to our manuscript titled, " Video Violence Recognition and Localization Using a Semi-Supervised Hard Attention Model." We were very encouraged by the reviewers' thoughtful, detailed, and challenging responses. We have thoroughly revised our manuscript based on your suggestions and comments. We address the comments made by the reviewers below:

\subsubsection*{\textbf{Reviewer \#1:}}

Thank you for carefully reviewing the paper. We have improved the paper based on your comment.

\hfill \break
\textbf{Comment 1:} \textit{“The manuscript needs an English proofreading.”}

The paper is edited by a professional native language editor (certificate attached). Multiple reviews have been conducted on the paper. It is our hope that the current language quality of the paper is up to your standards.


\subsubsection*{\textbf{Reviewer \#2:}}

Thank you for your insightful comments and your interest in our paper. Your comments have improved the quality of the revised paper. Responses to your points are as follows:

\hfill \break
\textbf{Comment 1:} \textit{“Firstly, the paper is not organized well.”}

In addition to updating the paper's format based on the Expert Systems With Applications Journal formatting, the paper has undergone a major contextual update. Many sections of the paper have been re-written, updated, and the logical flow of the paper has been streamlined.

\hfill \break
\textbf{Comment 2:} \textit{“The abstract is not convincing and is disorganized…”}

The abstract is rewritten based on your comments. As you have suggested, we have organized the paper’s abstract to state the problem and its relevance clearly. We have clearly stated the novelty and importance of the proposed method, followed by a summary of essential aspects of the SSHA model. And finally, the proposed method’s results are stated.

\begin{quote}
    \textbf{Problem statement and relevance:} \textit{“The significant growth of surveillance camera networks necessitates scalable AI solutions to efficiently analyze the large amount of video data produced by these networks. As a typical analysis performed on surveillance footage, video violence detection has recently received considerable attention. The majority of research has focused on improving existing methods using supervised methods, leaving semi-supervised approaches largely untouched.”}


    \textbf{Proposed method novelty and overview:} \textit{"In this study, a reinforcement learning model is introduced that can outperform existing models through a semi-supervised approach. The main novelty of the proposed method lies in the introduction of a semi-supervised hard attention mechanism. Using hard attention, the essential regions of videos are identified and separated from those that are irrelevant. A model's accuracy is improved by removing redundant data and focusing on useful visual information in a higher resolution. Implementing hard attention mechanisms using semi-supervised reinforcement learning algorithms eliminates the need for attention annotations in video violence datasets, thus making them readily applicable. The proposed model utilizes a pre-trained I3D backbone to accelerate and stabilize the training process."}

    \textbf{Proposed method results:} \textit{"The proposed model achieved state-of-the-art accuracy of 90.4\% and 98.7\% on RWF and Hockey datasets, respectively."}
\end{quote}

\hfill \break
\textbf{Comment 3:} \textit{“The tense used in sentences are not consistent”, “The whole text should be revised since there are misuses of words.”, “Please proof-read the whole text”}

A professional native English editor has edited the paper. We have especially emphasized the improvement of tense use and word usage in the text. In addition to the native proofreading, the text has undergone a significant rewrite to improve the text’s readability and flow. Thank you for taking the time to read the updated text. We hope it has addressed your concerns.

\hfill \break
\textbf{Comment 4:} \textit{“There are no citations for many sentences in this manuscript. Why? Please check”}

All sections have been checked for reference-less claims, and more than 14 instances have been identified (mainly in the introduction and related work sections). Relative and suitable references have been added to the paper.

\hfill \break
\textbf{Comment 5:} \textit{“The conclusions are not in accordance with the main problem originally stated.”}

Thank you for mentioning this error. The conclusions section is majorly updated to reflect the abstract's claims accurately. The reflecting parts of the conclusion are as follows:
    
\begin{quote}
    \textit{“This paper presents a semi-supervised hard attention mechanism (SSHA) based on reinforcement learning. SSHA achieves state-of-the-art accuracy in video violence detection by analyzing the most critical region of the video in greater depth. It utilizes video violence datasets that are readily available and eliminates the need for specialized datasets or annotations. The multi-stage implementation of SSHA enables the proposed model to utilize high-definition surveillance footage by selecting attention regions according to the user's preferences. The RGB-only version of the SSHA model achieved state-of-the-art 90.4 percent accuracy on the RWF dataset and 98.5 and 99.5 percent accuracy on the Hockey and Movies datasets, respectively.”}
\end{quote}


\subsubsection*{\textbf{Reviewer \#3:}}

Thank you for your detailed and in-depth comments and questions. We have incorporated the answer to your questions to improve the paper's details and quality. The following are the point-to-point responses to your comments:

\hfill \break
\textbf{Comment 1:} \textit{“In the process, authors have proposed a hard attention mechanism where the so called redundant information is completed removed…”}

The value of additional features is undeniable. They explicitly represent information that is not readily understandable in the raw RGB frames. Although hard attention could be used alongside the other features and is not a mutually exclusive replacement for the additional features, we suggest that hard attention is a more accessible and valuable alternative. As mentioned in the paper, the hard attention mechanism could be implemented without additional data or a larger neural network. In contrast, all additional features require different datasets, additional feature extraction computation, or additional neural streams.

Moreover, some additional information like skeleton estimation data are application-specific (work when the subject is the human body); hence are limited to the current application. In comparison, the hard attention assumption is to focus on the video's most important information. This assumption covers a broader range of applications as this assumption only relies on the existence of redundant information in data which is a common-place issue. In summary, besides mentioning these ideas throughout the paper in the revised version, we have explicitly added a paragraph in the methods \autoref{3:1}:

\begin{quote}
       \textit{“Compared to using the auxiliary features, the hard-attention methodology is more generalizable and cost-effective. In addition to the computational overhead of auxiliary features, some features, such as skeleton estimation, are selected based on the video violence detection application (importance of human body dynamics). Due to their application-specific nature, such features cannot be used in a broader range of computer vision applications. The low computational overhead and application-neutral assumptions of the hard attention mechanism make it suitable for a wider range of applications in computer vision.”}
\end{quote}
    

\hfill \break
\textbf{Comment 2:} \textit{“The evaluation measure is accuracy. Is this a good measure to evaluate the performance?...”}

We have added Table 3 to the paper. Table 3 shows the class-level performance of the SSHA model using precision, recall, and f1-score metrics. We have also added the total value of these metrics for all classes. As classes in the utilized datasets are perfectly balanced, the imbalance learning issues do not exist, and the class-level results are perfectly balanced. Unfortunately, the mentioned metrics are not available for the previous methods; hence a thorough class-level comparison of methods is not currently possible. However, such a comparison's importance is apparent and an exciting continuation of our research.

\hfill \break
\textbf{Comment 3:} \textit{“It is stated that Table 1 presents statistical comparison. This is misleading as the table provides some details about the data set”}
	
Thank you for mentioning the misleading caption. Table 1 caption is updated to \textit{“Video violence datasets characteristics.”}


\subsubsection*{\textbf{Reviewer \#5:}}

Thank you for your detailed, helpful, and insightful comments. Indeed, the topic at hand is interesting, and we have done our best to improve the quality of the paper based on your comments. The general steps done to apply your suggestions are as follows:

\begin{itemize}
    \item The paper has gone through a significant rewrite. All sections are rewritten, modified, or reorganized to improve the logical flow of the paper. Additionally, the paper is proofread by a professional native editor.
    
    \item We have tried to make our statements more explicit and clear. We have removed redundant information in the paper and tried emphasizing the main contributions and critical design elements. With these changes, we aim to clear a more coherent and clear picture of the proposed method and its applications in the reader’s mind.
    
    \item By explicitly mentioning the novelty of the presented research, especially in the abstract, introduction, discussion, and conclusion sections, we hope to conduct the novelty and originality of the study. In the revised version, we emphasized the paper's unique contributions by introducing the idea of a semi-supervised hard attention mechanism that is conceptualized, implemented, and evaluated in this research. By doing so, we tried to separate ourselves from non-original research in this field.  
\end{itemize}

The points to points response to your comments are as follows:

\hfill \break
\textbf{Comment 1:} \textit{“The abstract is vague and does not report any essential mechanism of the SSHA.”:}

The abstract is rewritten from scratch to reduce ambiguity. In the new abstract, we tried to focus on the paper's main contribution, which is the semi-supervised implementation of the hard attention mechanism using reinforcement learning. The updated abstract is organized as follows:

\begin{quote}
    \textbf{Problem context:} \textit{“The significant growth of surveillance camera networks necessitates scalable AI solutions to efficiently analyze the large amount of video data produced by these networks. As a typical analysis performed on surveillance footage, video violence detection has recently received considerable attention. The majority of research has focused on improving existing methods using supervised methods, leaving semi-supervised approaches largely untouched.”}

    \textbf{Summary of the semi-supervised hard attention method:} \textit{“In this study, a reinforcement learning model is introduced that can outperform existing models through a semi-supervised approach. The main novelty of the proposed method lies in the introduction of a semi-supervised hard attention mechanism. Using hard attention, the essential regions of videos are identified and separated from those that are irrelevant. A model's accuracy is improved by removing redundant data and focusing on useful visual information in a higher resolution. Implementing hard attention mechanisms using semi-supervised reinforcement learning algorithms eliminates the need for attention annotations in video violence datasets, thus making them readily applicable. The proposed model utilizes a pre-trained I3D backbone to accelerate and stabilize the training process.”}

    \textbf{Brief statement of results:} \textit{“The proposed model achieved state-of-the-art accuracy of 90.4\% and 98.7\% on RWF and Hockey datasets, respectively.”}
\end{quote}

\hfill \break
\textbf{Comment 2:} \textit{“It is not understood why the authors used BGR video frames instead of the standard RGB format…”}
	
Thank you for mentioning this issue. Using the BGR word creates a lot of confusion for the readers. As the OpenCV (our Python library of choice to read videos) library reads the image and video frames in BGR format, we have mentioned this format in the paper. However, the model itself uses RGB frames. To address your first concern, the conversion between BGR and RGB formats is very light-weighted. In fact, to replace the two blue and red channels, it is only needed to displace the pointers to those channels, which are two integer variables. This process is as simple as assigning a variable and could be done in a few nanoseconds. Additionally, we have used the RGB format throughout the model training and evaluation to keep the comparison with previous models fair. To address the ambiguity caused by mentioning the BGR format, we have replaced all usage of the BGR format with the RGB format.

\hfill \break
\textbf{Comment 3:} \textit{“Most of the parameters of the Eq1 are not defined. This also applies to Eq2, 3, and 4. Further, no references to Eq1 and 2.”}

To address this problem, we have added an explanation of the parameters and their relations after each equation. References to all equations are added. The equations are closer to their use in the text to increase the readability.

\hfill \break
\textbf{Comment 4:} \textit{“In the subsection "3.2 Design", what is a? Why a+1 is the correct selection, also why a-1 is the wrong selection? Why +0.5?”}

To address the first issue, the automated word spacing algorithm of latex software has put the article word “a” and the reward value “+1” and “-1” too close to each other. To avoid confusion, the paragraph is rewritten to remove the article word “a” before the reward values. Additionally, we have explained why we chose the +.5 value for the focus rewards. The +.5 value is not exact, and other values between 0 and 1 could have been used with similar results. This value should be larger than 0, as any reward less than 0 will encourage the model not to take that action. That is not our intention.

Moreover, as the reward for correct video classification is +1, should we choose a larger than +1 value for this reward, it would render the classification reward useless for the model as it would always select the larger reward. Hence, based on our experiments with different values for this reward, +.5 results in the best accuracy and training stability. The following explanation is added to the text to make this decision clear (\autoref{3:2}, paragraph 4):

\begin{quote}
    \textit{“The rewards are defined to be +1 for a correct video class selection and -1 for an incorrect class selection. Furthermore, a diminishing +0.5 reward is associated with attention action in order to encourage the reinforcement learning model to experiment with region selection. As rewards below 0 act as punishments, the auxiliary reward should be greater than 0 to encourage the model. Additionally, since the reward for a correct class selection is +1, the auxiliary reward must not overwhelm the primary reward by being more than +1. According to empirical analysis, values such as 0.3, 0.4, 0.5, and 0.7 result in reasonably similar results, with 0.5 being the best.”}
\end{quote}

\hfill \break
\textbf{Comment 5:} \textit{“In page 6, line 22: The authors mentioned that the predefined range is application and architecture-specific. However, I do not see this range in the evaluation part of this paper.”}
	
Thank you for mentioning this issue. We have added Figure 1 and its description to address this problem. The prior boxes are a few pre-defined and static regions on the model input, allowing the model to crop the input frame accordingly. Using these simple boxes, we can reduce the number of actions in each step, reducing the search space size of the reinforcement learning model. The reduced search space helps the model with faster and more stable training and convergence to an accurate solution. The following paragraph is a description of the prior boxes (\autoref{3:1}, paragraph 7):

\begin{quote}
    \textit{“The reinforcement learning environment utilizes predefined regions called prior boxes, as shown in \autoref{fig:priorbox}. Through the use of prior boxes, the model can focus on different regions of a video within one or more region selection stages. In each stage, the chosen area replaces the current frame; as a result, the rest of the inference is carried out using the chosen region. In this manner, the model may continue to tighten the attention region by selecting the most appropriate area at each subsequent iteration.”}
\end{quote}

Additionally, the following paragraph explains the reason we have used static and simple prior boxes (\autoref{3:1}, paragraph 10):

\begin{quote}
    \textit{“Selection of the region is accomplished by choosing from a set of prior boxes. Using static regions rather than a free-moving attention bounding box in the training phase reduces the search space for the deep reinforcement learning model. As opposed to the limited number of predefined prior bounding boxes, a free-moving attention bounding box can possess all the possible bounding boxes on the input image. Due to the limited number of sample videos in the video violence recognition datasets, reducing the reinforcement learning search space enhances the convergence and generalization of the learned network weights.”}
\end{quote}

\hfill \break
\textbf{Comment 6:} \textit{“Finally, the authors presented insufficient results for violence recognition, and no "actual" results are provided for the violence localization.”}
	
To complete the set of results provided for the violence recognition task, we have added the class-level and total precision, recall, and f1-score metrics in Table 3. The SSHA method achieved a 0.9 percent f1-score with a fair balance between precision and recall across the violent and non-violent classes. Additionally, to evaluate the effects of having the hard attention mechanism in the proposed method, we have evaluated the model with and without using the hard attention mechanism. Unfortunately, a more accurate evaluation of the hard attention mechanism using metrics like mAP is not possible currently, as the datasets in this field do not contain localization annotations. Hence, there is no ground truth to evaluate the localizations provided by the SSHA model. Yet, the increased accuracy of our model with the hard attention capability compared to the model without hard attention could be a good indication of its effectiveness.
